Generating Graphs via Spectral Diffusion

In this paper, we present GGSD, a novel graph generative model based on 1) the spectral decomposition of the graph Laplacian matrix and 2) a diffusion process. Specifically, we propose to use a denoising model to sample eigenvectors and eigenvalues from which we can reconstruct the graph Laplacian and adjacency matrix. Using the Laplacian spectrum allows us to naturally capture the structural characteristics of the graph and work directly in the node space while avoiding the quadratic complexity bottleneck that limits the applicability of other diffusion-based methods. This, in turn, is accomplished by truncating the spectrum, which, as we show in our experiments, results in a faster yet accurate generative process, and by designing a novel transformer-based architecture linear in the number of nodes. Our permutation invariant model can also handle node features by concatenating them to the eigenvectors of each node. An extensive set of experiments on both synthetic and real-world graphs demonstrates the strengths of our model against state-of-the-art alternatives.

==> immagini_mix.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.11\textwidth]{imgs/graph_planar_OURS_151.pdf}
  \includegraphics[width=0.11\textwidth]{imgs/graph_planar_OURS_122.pdf}
   \includegraphics[width=0.11\textwidth]{imgs/graph_planar_OURS_174.pdf}
    % \includegraphics[width=0.11\textwidth]{imgs/graph_planar_OURS_186.pdf}
    \caption{Graph samples produced by our model for the Planar dataset.}
    \label{fig:planar}
\end{figure}



\renewcommand{\CRB@setcopyrightparagraphstyle}{%
% Return to justifying text
\setlength{\rightskip}{0pt}
\setlength{\leftskip}{20pt}
}

\begin{figure}
    \centering
    
 
% \copyrightbox[l]{
% \includegraphics[width=0.1\textwidth]{imgs/graph_sbm_OURS_23.pdf}}{Generated Graphs}


 
\includegraphics[width=0.2\textwidth]{imgs/graph_sbm_OURS_23.pdf} \includegraphics[width=0.2\textwidth]{imgs/graphORI_planar_OURS_36.pdf}  



\includegraphics[width=0.2\textwidth]{imgs/graph_sbm_OURS_13.pdf}\includegraphics[width=0.2\textwidth]{imgs/graphORI_planar_OURS_5.pdf}   


\includegraphics[width=0.2\textwidth]{imgs/graph_sbm_OURS_70.pdf}   
\includegraphics[width=0.2\textwidth]{imgs/graphORI_sbm_OURS_85.pdf}  

\copyrightbox[b]{
\includegraphics[width=0.2\textwidth]{imgs/graph_sbm_OURS_31.pdf}  }{Generated Graphs}   \hfill \copyrightbox[b]{\includegraphics[width=0.2\textwidth]{imgs/graphORI_sbm_OURS_2_5comms.pdf}  }{Original Graphs}

% \copyrightbox[l]{
% \includegraphics[width=0.1\textwidth]{imgs/graphORI_planar_OURS_36.pdf}     }{Original Graphs}

 
   
            

         
    \caption{Graph visualization of some structures from the Stochastic Block Model dataset,  by  number of communities. Top row: graphs generated through our method. Bottom row: graphs from the training set. }
    
    \label{fig:sbm}
\end{figure}


% \makeatletter
\renewcommand{\CRB@setcopyrightparagraphstyle}{%
% Return to justifying text
\setlength{\rightskip}{0pt}
\setlength{\leftskip}{20pt}
}

\begin{figure}
    \centering\copyrightbox[b]{
    \includegraphics[width=0.2\textwidth]{imgs/graph_proteins_OURS_0_len_480.pdf}}{OURS - 480}
     \centering\copyrightbox[b]{
        \includegraphics[width=0.2\textwidth]{imgs/graph_proteins_test_788_len_484.pdf}}{ORI - 484}
         \centering\copyrightbox[b]{
              \includegraphics[width=0.2\textwidth]{imgs/graph_proteins_SPECTRE_92_len_481.pdf}}{SPECTRE - 481}
            \centering\copyrightbox[b]{
                      \includegraphics[width=0.2\textwidth]{imgs/graph_proteins_GraphRNN_148_len_480.pdf}}{GraphRNN - 480}
    \caption{Proteins}
    \label{fig:enter-label}
\end{figure}




==> tables/QM9_table.tex <==
\definecolor{Gray}{HTML}{E3E3E3}
\definecolor{LightGray}{HTML}{F4F4F4}
\newcolumntype{g}{>{\columncolor{LightGray}}c}

\begin{table}
\setlength{\tabcolsep}{0.65\tabcolsep}% Shrink \tabcolsep by 30%
\caption{QM9 dataset, molecule generation. Comparison with other graph generative models based on validity, uniqueness, and novelty metrics (the higher the better). 
Methods denoted by $^*$ are taken from   \cite{martinkus2022spectre}.TODO: digress loro numeri
\label{tab:qm9}} 
% Baseline results are taken from \cite{martinkus2022spectre}. spectre e graphvae da \cite{martinkus2022spectre} mentre digress lo abbiamo rifatto 
\scriptsize
\centering 
\ra{1.0} 
\begin{tabular}{@{}rccg@{}}
\toprule   & 
\multicolumn{3}{c}{\textbf{QM9} }       \\ 
\cmidrule{2-4}  
& Val.$\uparrow$&Val.\& Uniq.$\uparrow$&  Val.\& Uniq.\& Nov.$\uparrow$ \\
\midrule 
\midrule 
% GraphRNN &0.0000&0.0000&0.0000\\
% GRAN &0.0000&0.0000&0.0000\\
GraphVAE$^*$ & 0.5570 & 0.4200 & 0.2610 \\
DiGress$\;\,$ & 0.9900 & 0.9523 & \underline{0.3180}\\
GDSS & 0.8335 & 0.8281 & 0.7257 \\
SPECTRE$^*$ & 0.8730 & 0.3120 & 0.2910\\
\midrule
% \rowcolor{Gray}
\grasp$\;\,$ & 0.7430 & 0.5615 & \textbf{0.4531} \\
\bottomrule 
\end{tabular} 
\end{table}

==> tables/community_table.tex <==
 
\begin{table}

\setlength{\tabcolsep}{0.65\tabcolsep}% Shrink \tabcolsep by 30%
\caption{Community-small Dataset. Comparison with other graph generative models  using MMD metrics (the smaller the better). \label{tab:community} } 
\centering 
\ra{1.0} 
\begin{tabular}{@{}rrrrrr@{}}
\toprule   & 
\multicolumn{4}{c}{\textbf{Community-Small} }       \\ 
\cmidrule{2-5}  
& Deg. $\downarrow$ & Clus. $\downarrow$ & Spect. $\downarrow$  & Orb. $\downarrow$    \\
\midrule \midrule
 
GraphRNN &0.0271&0.1072&0.0520&0.1469  \\

GRAN & \textbf{0.0013} & {0.0843}& {0.0282}& {0.0201}  \\

DiGress & 0.0096 & 0.1035& 0.0506 & 0.0372   \\

\revised{GSDM} & 0.0099 & \textbf{0.0446} & \textbf{0.0131} & \underline{0.0155} \\

GDSS & 0.0107 & 0.1060 & 0.0450 & 0.0356 \\

SPECTRE & 0.0079 & 0.1067  & 0.0460  & 0.0250   \\

\midrule

{\grasp} &\underline{0.0016}& \underline{0.0590} & \underline{0.0153} & \textbf{0.0142}      \\


 
 
\bottomrule 
\end{tabular} 

\end{table}


% \begin{table}

% \setlength{\tabcolsep}{0.65\tabcolsep}% Shrink \tabcolsep by 30%
% \caption{Community-small Dataset. Comparison with other graph generative models  using MMD metrics (the smaller the better). \label{tab:community} } 
% \centering 
% \ra{1.0} 
% \begin{tabular}{@{}rrrrrr@{}}
% \toprule   & 
% \multicolumn{4}{c}{\textbf{Community-Small} }       \\ 
% \cmidrule{2-5}  
% & Deg. $\downarrow$ & Clus. $\downarrow$ & Spect. $\downarrow$  & Orb. $\downarrow$    \\
% \midrule \midrule
 
% GraphRNN &0.02711&0.10725&0.05196&0.14682  \\

% GRAN & \textbf{0.00135} & {0.08427}& {0.02816}& {0.02013}  \\

% DiGress & 0.00964 & 0.10351& 0.05065 & 0.03721    \\

% GSDM & 0.00993 & \textbf{0.04458} & \textbf{0.01310} & \underline{0.01553} \\

% GDSS & 0.01071 & 0.10601 & 0.04492 & 0.03556 \\

% SPECTRE & 0.00786 & 0.10669  & 0.04597  & 0.02495   \\

% \midrule

% {\grasp} &\underline{0.00160}& \underline{0.05900} & \underline{0.01528} & \textbf{0.01426}      \\


 
 
% \bottomrule 
% \end{tabular} 

% \end{table}



% \definecolor{LightGray}{HTML}{F4F4F4}
% \newcolumntype{g}{>{\columncolor{LightGray}}c}

% \begin{table}
% \setlength{\tabcolsep}{0.65\tabcolsep}% Shrink \tabcolsep by 30%
% \caption{Community over Big} 
% \centering 
% \ra{1.0} 
% \begin{tabular}{@{}rrrrrg@{}}
% \toprule   & 
% \multicolumn{5}{c}{\textbf{Community Small} }       \\ 
% \cmidrule{2-6}  
% & Deg. $\downarrow$ & Clus. $\downarrow$ & Spect. $\downarrow$  & Orb. $\downarrow$  & Ratio \\
% \midrule \midrule
% \textit{Training}   &  0.00238 & 0.01843 & 0.00633  & 0.00429  &    
% \\
% \midrule 
% GraphRNN &0.02711&0.10725&0.05196&0.14682& \\

% GRAN & \textbf{0.00135} & 0.08427&0.02816& 0.02013& \\

% DiGress & 0.00964 & 0.10351& 0.05065 & 0.03721 &  \\


% SPECTRE & 0.00786 & 0.10669  & 0.04597  & 0.02495&  \\

% \midrule

% OUR &0.00160& \textbf{0.05900} & \textbf{0.01528} & \textbf{0.01426}&     \\


 
 
% \bottomrule 
% \end{tabular} 

% \end{table}

==> tables/planar_table.tex <==
\definecolor{LightGray}{HTML}{F4F4F4}
\newcolumntype{g}{>{\columncolor{LightGray}}c}

\begin{table}

\setlength{\tabcolsep}{0.65\tabcolsep}% Shrink \tabcolsep by 30%
\caption{Planar dataset.  
Comparison with other graph generative models using MMD metrics (the smaller the better).% We were unable to replicate the results reported for SPECTRE in~\cite{martinkus2022spectre} by using the code provided by the authors on GitHub.  
\label{tab:planar}} 
\centering 
\ra{1.0} 
\begin{tabular}{@{}rrrrrg@{}}
\toprule   & 
\multicolumn{4}{c}{\textbf{Planar Graphs}}       \\ 
\cmidrule{2-5}  
& Deg. $\downarrow$ & Clus. $\downarrow$ & Spect. $\downarrow$  & Orb. $\downarrow$   \\
\midrule 
\midrule 


GraphRNN & 0.0096 & 0.2985 & 0.0389 & 1.4022 \\

GRAN & 0.0202 & 0.2985 & 0.0248 & 0.1964 \\

DiGress & \textbf{0.0005} & \textbf{0.0178} & \textbf{0.0020} & \underline{0.0115} \\

\revised{GSDM} & 0.0220 & \underline{0.0222} & 0.0096 & 0.0371 \\

GDSS & 0.0701 & 0.3025 & 0.0403 & 1.0345 \\

% SPECTRE* & 0.2982 & 0.3386 & 0.1329 & 1.6817    \\

% SPECTRE new ckpt & 0.0008 & 0.0691 & 0.0051 & 0.0033 \\

SPECTRE & 0.0008 & 0.08585 & 0.01474 & 0.00578 \\

\midrule

\grasp & \underline{0.0012} & {0.1881} & \underline{0.0057} & \textbf{0.0047} \\

\bottomrule 
\end{tabular} 
\end{table}

% \definecolor{LightGray}{HTML}{F4F4F4}
% \newcolumntype{g}{>{\columncolor{LightGray}}c}

% \begin{table}
% \setlength{\tabcolsep}{0.65\tabcolsep}% Shrink \tabcolsep by 30%
% \caption{Planar over Big} 
% \centering 
% \ra{1.0} 
% \begin{tabular}{@{}rrrrrg@{}}
% \toprule   & 
% \multicolumn{5}{c}{\textbf{Planar Graphs} }       \\ 
% \cmidrule{2-6}  
% & Deg. $\downarrow$ & Clus. $\downarrow$ & Spect. $\downarrow$  & Orb. $\downarrow$  & Ratio \\
% \midrule 
% \midrule 
% \textit{Training}   &0.00009 & 0.00579& 0.00069&0.00162 &  
% \\
% \midrule   
% GraphRNN & 0.00959 & 0.29855  & 0.03891 &1.40225& \\

% GRAN &  0.02020 & 0.29848  & 0.02480 &0.19644 & \\

% DiGress & 0.00050 & \textbf{0.01783} & \textbf{0.00203} &  0.01152 &  \\

% SPECTRE & \grey{0.00038} & \grey{0.05261}  & \grey{0.00567}  & \grey{0.00143} &  \\

% \midrule

% OUR & 0.00125 & 0.18809  & 0.00572&0.00469 &     \\
 
% \bottomrule 
% \end{tabular} 

% \end{table}

==> tables/sbm_table.tex <==

\begin{table}

\setlength{\tabcolsep}{0.65\tabcolsep}% Shrink \tabcolsep by 30%
\caption{ Stochastic Block Model dataset. Comparison with other graph generative models using MMD metrics (the smaller the better).   \label{tab:SBM}} 
\centering 
\ra{1.0} 
\begin{tabular}{@{}rrrrrg@{}}
\toprule & 
\multicolumn{4}{c}{\textbf{Stochastic Block Model} } \\ 
\cmidrule{2-5}  
& Deg. $\downarrow$ & Clus. $\downarrow$ & Spect. $\downarrow$ & Orb. $\downarrow$ \\
\midrule 
\midrule 

GraphRNN & 0.0178 & 0.0151 & 0.0104 & 0.0351 \\

GRAN & 0.0135  & 0.0149 & \underline{0.0034} & 0.0352 \\

DiGress & 0.0166 & 0.0246 & 0.0064 & 0.1327 \\

\revised{GSDM} & 0.2295 & 0.2280 & 0.1578 & 0.2876 \\

GDSS & 0.2658 & 0.0442 & 0.0551 & 0.2780 \\

SPECTRE & \underline{0.0044} & \underline{0.0118} & \textbf{0.0015} & \textbf{0.0140} \\

\midrule
\grasp & \textbf{0.0005} & \textbf{0.0115} & 0.0045 & \underline{0.0289} \\

 
\bottomrule 
\end{tabular} 

\end{table}

% \begin{table}

% \setlength{\tabcolsep}{0.65\tabcolsep}% Shrink \tabcolsep by 30%
% \caption{ Stochastic Block Model dataset. Comparison with other graph generative models using MMD metrics (the smaller the better).   \label{tab:SBM}} 
% \centering 
% \ra{1.0} 
% \begin{tabular}{@{}rrrrrg@{}}
% \toprule & 
% \multicolumn{4}{c}{\textbf{Stochastic Block Model} } \\ 
% \cmidrule{2-5}  
% & Deg. $\downarrow$ & Clus. $\downarrow$ & Spect. $\downarrow$ & Orb. $\downarrow$ \\
% \midrule 
% \midrule 

% GraphRNN & 0.01784 & 0.01515 & 0.01040 & 0.03513 \\

% GRAN & 0.01348  & 0.01488 & \underline{0.00342} & 0.03516 \\

% DiGress & 0.01656 & 0.02459 & 0.00644 & 0.13271 \\

% Fast & 0.22950 & 0.22799 & 0.15785 & 0.28765 \\

% GDSS & 0.26583 & 0.04421 & 0.05515 & 0.27802 \\

% SPECTRE & \underline{0.00444} & \underline{0.01184} & \textbf{0.00150} & \textbf{0.01399} \\

% \midrule
% \grasp & \textbf{0.00055} & \textbf{0.01152} & 0.00454 & \underline{0.02890} \\

 
% \bottomrule 
% \end{tabular} 

% \end{table}








% \definecolor{LightGray}{HTML}{F4F4F4}
% \newcolumntype{g}{>{\columncolor{LightGray}}c}

% \begin{table}
% \setlength{\tabcolsep}{0.65\tabcolsep}% Shrink \tabcolsep by 30%
% \caption{ Sbm over Big} 
% \centering 
% \ra{1.0} 
% \begin{tabular}{@{}rrrrrg@{}}
% \toprule   & 
% \multicolumn{5}{c}{\textbf{Stochastic Block Model} }       \\ 
% \cmidrule{2-6}  
% & Deg. $\downarrow$ & Clus. $\downarrow$ & Spect. $\downarrow$  & Orb. $\downarrow$  & Ratio \\
% \midrule 
% \midrule 
% \textit{Training}     & 0.00040& 0.01284 &0.01440 & 0.00142&
% \\
% \midrule 
% GraphRNN  & 0.01784 & 0.01515  & 0.01040 & 0.03513   &\\

% GRAN  &0.01348  & 0.01488 & {0.00342}& 0.03516 &   \\

% DiGress &   0.01656  & 0.02459 & 0.00644&0.13271&\\


% SPECTRE &  0.00444 & \textbf{0.01124} &\textbf{0.00150}    & \textbf{0.01399}&\\

%  \midrule
% OUR &\textbf{0.00067}& 0.01660& 0.01238 & 0.03387&\\

 
% \bottomrule 
% \end{tabular} 

% \end{table}
